Algorithmic Extensions of Dirac's Theorem

In 1952, Dirac proved the following theorem about long cycles in graphs with large minimum vertex degrees: Every $n$-vertex $2$-connected graph $G$ with minimum vertex degree $\delta\geq 2$ contains a cycle with at least $\min\{2\delta,n\}$ vertices. In particular, if $\delta\geq n/2$, then $G$ is Hamiltonian. The proof of Dirac's theorem is constructive, and it yields an algorithm computing the corresponding cycle in polynomial time. The combinatorial bound of Dirac's theorem is tight in the following sense. There are 2-connected graphs that do not contain cycles of length more than $2\delta+1$. Also, there are non-Hamiltonian graphs with all vertices but one of degree at least $n/2$. This prompts naturally to the following algorithmic questions. For $k\geq 1$, (A) How difficult is to decide whether a 2-connected graph contains a cycle of length at least $\min\{2\delta+k,n\}$? (B) How difficult is to decide whether a graph $G$ is Hamiltonian, when at least $n - k$ vertices of $G$ are of degrees at least $n/2-k$? The first question was asked by Fomin, Golovach, Lokshtanov, Panolan, Saurabh, and Zehavi. The second question is due to Jansen, Kozma, and Nederlof. Even for a very special case of $k=1$, the existence of a polynomial-time algorithm deciding whether $G$ contains a cycle of length at least $\min\{2\delta+1,n\}$ was open. We resolve both questions by proving the following algorithmic generalization of Dirac's theorem: If all but $k$ vertices of a $2$-connected graph $G$ are of degree at least $\delta$, then deciding whether $G$ has a cycle of length at least $\min\{2\delta +k, n\}$ can be done in time $2^{\mathcal{O}(k)}\cdot n^{\mathcal{O}(1)}$. The proof of the algorithmic generalization of Dirac's theorem builds on new graph-theoretical results that are interesting on their own.

==> path-1-connected.tex <==
\section{Finding paths in non-biconnected graphs}





	\begin{lemma}\label{lemma:path_from_cut_vertex}
	Let $G$ be a connected separable graph with a given subset of its vertices $B$.
	Let $0<k \le\frac{1}{3}\delta(G - B)$ be an integer.
	Let $H$ be a non-leaf block of $G$ that contains a path of length $k+|B|$ starting in a cut vertex.
	Then $H$ contains a path of length at least $k$ between two cut vertices.
\end{lemma}
\begin{proof}
	Let $c$ be a starting cut vertex of the path from the problem statement.
	While the path ends with a vertex in $B$ or contains more than $k+1$ vertices outside $B$, remove the last edge from the path.
	We obtain a path of length at least $k$ and at most $k+|B|$ starting in $c$ and ending in $v \notin B$.
	If $v$ is a cut vertex, we are done.
	Otherwise, the degree of $v$ in $H$ is at least $\delta(G-B)$.
	Consider a graph obtained from $H$ with deleting all vertices of the path ending in $v$, except $v$.
	Denote by $C$ the connected component of $v$ in this graph.
	
	If $C$ contains at least one cut-vertex of the initial graph $G$, then we are done, as we can append the path between $v$ and this cut-vertex to the initial path.
	Now $C$ does not contain any cut vertex of $G$, so  $\delta(H[C]-B)\ge\delta(G-B)-k\ge 2k$, as the path between $c$ and $v$ contains at most $k+1$ vertices (including $v$) outside $B$.
	If $H[C]$ is biconnected, then by Theorem~\ref{thm:relaxed_long_cycle} there is a cycle of length at least $\delta(H[C]-B)\ge 2k$ in $H[C]$, and we are done by Lemma~\ref{lemma:biconnected_cycle_to_any_path}.
	If the $B$-refinement of $H[C]$ is biconnected, apply the same argument to the $B$-refinement of $H[C]$ to show that there is a cycle of length at least $2k$ in $H$.
	
	It is left to consider the case when neither $H[C]$ nor its $B$-refinement $R(H[C],B)$ are biconnected.
	Note that $\delta(R(H[C],B)-B)=\delta(H[C]-B)\ge 2k$.
	Consider a leaf-block $L$ of $R(H[C],B)$.
	Denote the cut vertex of $L$ by $u$.
	As a part of a $B$-refinement, $L$ contains at least one inner vertex outside $B$.
	Its degree is at least $2k$, so $L$ consists of at least $2k+1\ge 3$ vertices, so $L$ is biconnected.
	Note that $\delta(L-(B\cup\{u\}))\ge 2k-1$, so by Theorem~\ref{thm:relaxed_long_cycle} $L$ contains a cycle on at least $2k-1$ vertices.
	Finish with Lemma~\ref{lemma:biconnected_cycle_to_any_path} as before.
\end{proof}

\begin{lemma}\label{lemma:long_block_path}
	Let $G$ be a connected separable graph with a given subset of its vertices $B$.
	Let $0<k \le\frac{1}{3}\delta(G - B)$ be an integer.
	If there is a path of length at least $2(k+|B|)$ that is fully contained in any non-leaf block of $G$, then there is a path of length at least $k$ between some pair of distinct cut vertices of $G$.
\end{lemma}
\begin{proof}
	Take any cut-vertex of the block and build a path that connects it with the closest vertex on the path of length at least $2(k+|B|)$.
	This closest vertex splits the path onto two parts, remove the smallest of them.
	This yields a path of length at least $k+|B|$ starting in a cut-vertex.
	Finish using the previous lemma.
\end{proof}

\begin{lemma}\label{lemma:large_leafblocks}
	Let $G$ be a connected separable $B$-refined graph and $k\le \delta(G-B)-4$ be a positive integer.
	Let $L_1, L_2$ be two-distinct leaf-blocks of $G$.
	If $|V(L_1)\setminus B|+|V(L_2)\setminus B|\ge 2\delta(G-B)+k+4$, then there is a path of length at least $2\delta(G-B)+k$ in $G$.
\end{lemma}
\begin{proof}
	Denote the cut vertex of $L_i$ by $c_i$.
	Since $G$ is $B$-refined, at least one inner vertex in each leaf block is outside $B$, so $\delta(L_i - (B\cup\{c_i\}))\ge \delta(G-B)-1$ for $i\in \{1,2\}$.
	By Corollary~\ref{thm:relaxed_st_path}, for each $i \in \{1,2\}$ there is a path of length at least $\delta(G-B)-1$ inside $L_i$ starting in $c_i$, where $c_i$ denotes the cut vertex of $L_i$.

	Now assume that $|V(L_1)\setminus B|\ge 2\delta(G-B)-1$.
	By Theorem~\ref{thm:relaxed_long_cycle}, there is a cycle in $L_1$ of length at least $2\delta(L_1-(B\cup\{c_1\}))\ge 2\delta(G-B)-2$.
	Then there is a path in $L_1$ ending in $c_1$ of length at least $2\delta(G-B)-3$.
	Combine this path with a path of length $\delta(G-B)-1$ inside $L_2$ starting in $c_2$ using any path between $c_1$ and $c_2$.
	The obtained path is of length at least $3\delta(G-B)-4\ge 2\delta(G-B)+k$.
	The case $|V(L_2)\setminus B|\ge 2\delta(G-B)-1$ is symmetrical.
	
	It is left to consider the case when $|V(L_1)\setminus B|, |V(L_2)\setminus B| < 2\delta(G-B)-1$.
	By Theorem~\ref{thm:relaxed_long_cycle}, there is a cycle of length at least $|V(L_i)\setminus (B\cup\{c_i\})|$ in $L_i$ for each $i \in \{1,2\}$.
	Hence, there is a path inside $L_i$ of length at least $|V(L_i)\setminus B|-2$ starting in $c_i$.
	Combine the paths for $i=1$ and $i=2$ into a single path of length at least $(|V(L_1)\setminus B|-2)+(|V(L_2)\setminus B|-2)\ge 2\delta(G-B)+k$.
\end{proof}



\begin{lemma}\label{lemma:path_between_cut_vertices_to_long_path}
	Let $G$ be a connected separable $B$-refined graph.
	If there is a path of length at least $k+2$ between any two distinct cut-vertices of $G$, then there is a path of length at least $2\delta(G-B)+k$ in $G$ starting and ending with edges of different leaf-blocks.
\end{lemma}
\begin{proof}
	By Corollary~\ref{thm:relaxed_st_path}, any leaf-block of a $B$-refinement contains a path of length at least $\delta(G-B)-1$ starting in its cut vertex.
	Thus, if a path from the lemma statement exists, one can extend it to a path between cut vertices of distinct leaf-blocks and combine it with two long paths inside them starting in the cut vertices.
\end{proof}

\begin{lemma}
	Let $G$ be a connected separable $B$-refined graph and let $k$ be a positive integer, such that $k+2 \le \frac{1}{3}\delta(G-B)$ and $2(k+2+|B|)\le \delta(G-B)$.
	If there is no path of length at least $2\delta(G-B)+k$ in $G$ that starts and ends with leaf-block edges of different blocks, then there is no path of length at least $\delta(G-B)+3k+6+2|B|$ in $G$ that does not start or end with a leaf-block edge or is contained in a leaf-block of $G$.
\end{lemma}
\begin{proof}
	The proof is by contradiction.
	Suppose that there is a path of length at least $\delta(G-B)+3k+6+2|B|$ in $G$ that does not end with a leaf-block edge.
	We show how to construct a path of length at least $2\delta(G-B)+k$ starting and ending in inner vertices of different leaf-blocks of $G$.
	
	If the path does not contain any cut-vertex, then it is fully contained in some non-leaf-block.
	Since $\delta(G-B)+3k+6+2|B|> 2(k+2+|B|)$, we obtain a path of length at least $k+2$ between some pair of cut-vertices of $G$ by Lemma~\ref{lemma:long_block_path} and finish with Lemma~\ref{lemma:path_between_cut_vertices_to_long_path}.
	If the path does contain at least one cut-vertex of $G$, then there is a path of length at least $\frac{1}{2}\delta(G-B)+\frac{3}{2}k+3+|B|> 2k+3+|B|$ starting in a cut-vertex of $G$.
	If this path contains no other cut-vertex of $G$, then we are done by Lemma~\ref{lemma:path_from_cut_vertex}.
	Otherwise, consider the last cut-vertex on this path.
	If it is on the distance at least $k+2$ from the start, we obtain the required path between cut vertices for Lemma~\ref{lemma:path_between_cut_vertices_to_long_path}.
	Otherwise, remove the part of the path from the start to this cut-vertex and obtain a path of length at least $(2k+3+|B|)-(k+1)= k+2+|B|$ starting in a cut vertex.
	Apply Lemma~\ref{lemma:path_from_cut_vertex} and Lemma~\ref{lemma:path_between_cut_vertices_to_long_path} to this path.
	
	Now assume that the path starts with an edge of a leaf-block $L$ of $G$, but ends with an edge of some non-leaf-block.
	If $|V(L)\setminus B|> \delta(G-B)+k+2$, then take any other leaf-block $L'$ of $G$ and apply Lemma~\ref{lemma:large_leafblocks} to $L$ and $L'$.
	Note that $|V(L')\setminus B| \ge \delta(G-B)+1$ holds since $L'$ contains at least one inner vertex outside $B$.
	
	It is left to consider the case when $|V(L)\setminus B|\le \delta(G-B)+k+2$.
	Then our path cannot contain more than $|L|-1\le \delta(G-B)+k+1+|B|$ edges inside $L$.
	Remove all edges inside $L$ from the path.
	The obtained path is a path of length at least $(\delta(G-B)+3k+6+2|B|)-(\delta(G-B)+k+1+|B|)>2k+3+|B|$ that starts in a cut vertex of $G$ and does not contain any leaf-block edge.
	We already considered this case before.
	
	If the path is completely contained in some leaf-block of $G$, then we obtain a leaf-block $L$ with $|V(L)\setminus B|> \delta(G-B)+k+2$.
	This case was also considered before.
\end{proof}

\begin{theorem}\label{thm:long_dp_separable_main}
	Let $G$ be a graph with subset of its vertices $B\subseteq V(G)$ such that $R(G,B)$ is connected but separable.
	Let $k>0$ be a given integer such that $3(k+2+|B|)\le \delta(G-B)$.
	If $G$ contains a path of length at least $2\delta(G-B)+k$, then $G$ contains a path of length at least $2\delta(G-B)+k$ that starts with zero or more edges in $E(G)\setminus E(R(G,B))$, then goes from an inner vertex of a leaf-block of $R(G,B)$ to an inner vertex of another leaf-block of $R(G,B)$, and ends with zero or more edges in $E(G)\setminus E(R(G,B))$. 
\end{theorem}
\begin{proof}
	Denote $H:=R(G,B)$.
	Assume there is a path of length at least $2\delta(G-B)+k$ in $G$.
	If this path consists completely of edges of $H$, then the required path exists by the previous lemma.
	Hence, this path starts in some vertex $b \in B\setminus V(H)$ with an edge in $E(G)\setminus E(H)$.
	Moreover, we can assume that there is no required path of length at least $2\delta(G-B)+k$ in $H$.
	
	Note that if the path does not contain any edge of $H$, then its length cannot be greater than $|B|<\delta(G-B)$, so it necessary contains at least one edge in $E(H)$.
	Hence, our path starts in the vertex $b$, then goes to a vertex $s \in V(H)$, and then goes only through the vertices of $H$ to some vertex $t \in V(H)$.
	The vertex $t$ is either the last vertex on the path, or the next vertex on the path is a vertex from $B\setminus V(H)$, and the rest of the path consists of edges outside $H$.
	Nevertheless, $t$ is the last vertex from $V(H)$ on the path.
	
	We have a path between $s$ and $t$ of length at least $2\delta(G-B)+k-|B|>\delta(G-B)+3k+6+2|B|$ inside $H$.
	If $s$ and $t$ are not both inner vertices of different leaf-blocks of $H$, then $H$ contains the required path by the previous lemma, which is a contradiction.
	The proof is complete.
\end{proof}

\begin{theorem}
	\probDP is solvable in $2^{\Oh(k+|B|)}\cdot \polyn$ running time, when the $B$-refinement of $G$ is connected but separable.
\end{theorem}
\begin{proof}
	The algorithm solving the problem is presented in Algorithm~\ref{alg:ldp_separable}.
	It is self-explanatory, so we analyze its correctness and running time.
	We note that $2\delta(G-B)<|V(G)|-|B|$ always holds for input instances of \textsc{\probDP in Separable Graphs}.

	\begin{algorithm}[ht]
		\KwIn{an instance $(G,B,k)$ of \textsc{\probDP in Separable Graphs}}
		\KwResult{\textsc{Yes} or \textsc{No} depending on whether $(G,B,k)$ is a yes-instance or a no-instance}
		\SetKwFunction{LongestPath}{longest\_path}%%
		\SetKwFunction{LongSTPath}{long\_st\_path}%%
		\SetKwFunction{LongErdosSTPath}{long\_eg\_st\_path}%%
		\If{$3(k+2+|B|)>\delta(G-B)$}{
			\Return{\LongestPath$(G,2\delta(G-B)+k)$}
		}
		\If{$2\delta(G-B)+k\ge n$}{
			\Return{\textsc{No}}
		}
		\If{$k=0$ and $|B|=0$}{
			\Return{\textsc{Yes}}
		}
		$H \longleftarrow R(G,B)$
		
		\ForEach{leaf-block $L$ of $H$}{
			\If{$|V(L)\setminus B|> \delta(G-B)+k+2$}{
				\Return{\textsc{Yes}}
			}
		}
	
		$G' \longleftarrow (V(G), E(G)\setminus E(H))$
		
		\ForEach{distinct leaf-blocks $L_1, L_2$ of $H$}{
			$c_1, c_2 \longleftarrow$ cut vertices of $L_1$ and $L_2$

			\ForEach{$s_1 \in V(L_1)\setminus \{c_1\}$ and $s_2 \in V(L_2)\setminus \{c_2\}$}{
				\ForEach{$i \in \{1,2\}$}{
					$b_i \longleftarrow 0$
					
					\ForEach{$v \in B$}{
						\While{\LongSTPath$(G',s_i,v,b_i+1)$ is \textsc{Yes}}{
							$b_i \longleftarrow b_i+1$
						}
					}
					
					$k_i \longleftarrow 0$
					
					\While{\LongErdosSTPath$(L_i, \{c_i\}\cup (B\cap V(L_i)), s_i, c_i,k_i+1)$ is \textsc{Yes}}{$k_i\longleftarrow k_i+1$}
					
					$d_i \longleftarrow b_i+\delta(L_i-(B\cup\{c_i\}))+k_i$
				}
			
				\If{\LongSTPath$(H,c_1, c_2,\max\{0,(2\delta(G-B)+k)-(d_1+d_2)\})$}{
					\Return{\textsc{Yes}}
				}
			}
		}

		\Return{\textsc{No}}
		\caption{Algorithm solving \probDP on separable graphs.}
		\label{alg:ldp_separable}
	\end{algorithm}

	If $3(k+2+|B|)>\delta(G-B)$, then the algorithm just employs the standard color-coding algorithm for \textsc{Longest Path} to find the required path.
	It runs in $2^{\Oh(k+|B|)}\cdot \polyn$ time.
	A simple path in an $n$-vertex graph cannot have length greater than $n-1$, so if $2\delta(G-B)+k\ge n$, the algorithm decides that the given instance is a no-instance.
	The condition $k=|B|=0$ corresponds to a yes-instance according to Theorem~\ref{thm:relaxed_long_path}.
	Here the assumption that $G$ is connected follows from that $R(G,B)$ is connected.
	
	Then the algorithm puts $H:=R(G,B)$, and here we can be sure that $|V(H)|>6$ and assume that $H$ is connected but separable.
	Moreover, $H$ is found in time polynomial in $n$.
	The next part of the algorithm checks if there is any leaf-block in $H$ consisting of too many vertices outside $B$.
	If such a leaf-block exists, then $(G,B,k)$ is clearly a yes-instance by means of Lemma~\ref{lemma:large_leafblocks}.
	
	The last part of the algorithm starts from finding the graph $G'$, which consists of edges of $G$ outside $H$.
	Note that each edge in $G'$ has at least one endpoint in $B$, so each connected component in $G'$ is of size at most $|B|+1$.
	Then the algorithm iterates over each pair of distinct leaf-blocks in $H$ and each pair of inner vertices inside them, which comprises a polynomial number of options.
	For each such fixed pair $s_1, s_2$, the algorithm tries to find a path described in the statement of Theorem~\ref{thm:long_dp_separable_main}: it starts with edges of $G'$, then goes from $s_1$ to the cut vertex $c_1$, then goes from $c_1$ to $c_2$, then from $c_2$ to $s_2$ inside $H$, and finally ends with edges of $G'$.
	The numbers $b_1$ and $b_2$ correspond to the maximum possible number of edges from $G'$ respectively in the start and in the end of the path.
	Each $b_i$ is found in $2^{\Oh(|B|)}\cdot\polyn$ running time with color-coding, as $G'$ contains no path longer than $|B|$.
	
	The values $k_i$ describe the length of the longest path from $s_i$ to $c_i$.
	By Corollary~\ref{thm:relaxed_st_path}, this path is of length at least $\delta(G-(B\cup\{c_i\}))\ge \delta(G-B)-1$, so its length can be described in the form $\delta(G-(B\cup \{c_i\}))+k_i$ for integer $k_i\ge 0$.
	On the other hand, the length of this path is at most $|V(L_i)|-1\le \delta(G-B)+k+|B|-1$, so $k_i \le k+|B|$.
	Thus, using the algorithm of Theorem~\ref{thm:long_eg_st_path_algo} for \probstP, the value of $k_i$ can be found in $2^{\Oh(k+|B|)}\cdot\polyn$ running time.
	The value of $d_i$ is the sum of $b_i$ and the longest path between $s_i$ and $c_i$.
	
	The last part of the path is the longest path between $c_1$ and $c_2$, and it is enough for the algorithm to check that it is long enough to decide that $(G,B,k)$ is a yes-instance.
	Note that the value of $(2\delta(G-B)+k)-(d_1+d_2)$ is at most $k+2$, so the check is done in $2^{\Oh(k)}\cdot \polyn$ running time.
	
	If no path is found, the algorithm decides that $(G,B,k)$ is a no-instance.
	This decision is clearly correct by Theorem~\ref{thm:long_dp_separable_main}.
	The total running time of the algorithm is $2^{\Oh(k+|B|)}\cdot\polyn$.
	This finishes the proof.	
\end{proof}

==> path-altogether.tex <==
\section{Long Dirac Path}\label{sec:longDiracPath}

\todo[backgroundcolor=yellow,inline]{this section describes reduction from cycle to path and probably is not needed}
\begin{comment}
In this section, we prove Theorem~\ref{theorem:main_path}.
The proof crucially relies on the following lemma.

\begin{lemma}\label{lemma:main_lemma_path}
	Let $G$ be a $2$-connected graph and $B\subseteq V(G)$ be a subset of its vertices such that $\delta(G-B)\ge 5$.
	Let $C$ be a cycle of length at least $2\delta(G-B)$ in $G$ and let $k< \frac{2}{5}\delta(G-B)$ be a non-negative integer.
	There is an algorithm that in polynomial time finds either:
	\begin{itemize}
		\item Longer cycle in $G$, or
		\item Path of length at least $2\delta(G-B)+k$ in $G$, or
		\item Vertex cover of $G-B$ of size at most $\delta(G-B)+2k$.
	\end{itemize}
\end{lemma}
\begin{proof}
	\todo[inline,backgroundcolor=yellow]{write this proof}
\end{proof}


\begin{proof}[Proof of Theorem~\ref{theorem:main_path}]
	\todo[backgroundcolor=yellow]{this is very sketchy}
	We assume that $G$ is connected, otherwise we apply the algorithm to each of its connected components.
	If the $B$-refinement of $G$ is not $2$-connected, apply the algorithm for \textsc{\probDP in Separable Graphs}.
	Otherwise, apply algorithm of Lemma~\ref{lemma:main_lemma_path} exhaustively to $(G,B,k)$ while the longer cycle is found.
	If the length of the cycle is at least $2\delta(G-B)+k+1$ or a path of length at least $2\delta(G-B)+k$ is found by this algorithm, we can decide that the input instance is a yes-instance.
	Otherwise, we obtain a vertex cover of the initial graph $G$ that is of size at least $2k+|B|$ and contains $B$ as a subset.
	Finish using the FPT-algorithm for \textsc{\probDC/Vertex Cover Above Degree}.
\end{proof}
\end{comment}
